Towards AI-driven Sign Language Generation with Non-manual Markers

Sign languages are essential for the Deaf and Hard-of-Hearing (DHH) community. Sign language generation systems have the potential to support communication by translating from written languages, such as English, into signed videos. However, current systems often fail to meet user needs due to poor translation of grammatical structures, the absence of facial cues and body language, and insufficient visual and motion fidelity. We address these challenges by building on recent advances in LLMs and video generation models to translate English sentences into natural-looking AI ASL signers. The text component of our model extracts information for manual and non-manual components of ASL, which are used to synthesize skeletal pose sequences and corresponding video frames. Our findings from a user study with 30 DHH participants and thorough technical evaluations demonstrate significant progress and identify critical areas necessary to meet user needs.

==> fig_tab/confusion_matrix.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/confusion_matrix.png}
    \caption{Confusion Matrix for Each Type. \han{TODO: update this once we manually label the test set}}
    \label{fig:data_prep}
\end{figure}

==> fig_tab/demographics.tex <==
\begin{table}[htb!]
    \caption{User Demographics and Language Proficiency.}
    \label{tab:demo}
    \centering
 \renewcommand{\arraystretch}{1.05}
\resizebox{0.85\textwidth}{!}{\begin{tabular}{llllllll}
        \toprule
        \hline
        PID & Gender & Age & Learned ASL Age & \makecell[c]{ASL Proficiency} & English Proficiency & \makecell[c]{ASL Use \\ Frequency}  & \makecell[c]{English Use \\ Frequency} \\\hline
        P1 & & & & & &  \\
        \rowcolor[HTML]{EFEFEF} P2 & & & & & &  & \\
        P3 & & & & & & & \\
        \rowcolor[HTML]{EFEFEF} P4 & & & & & & & \\
        P5 & & & & & & & \\
        \rowcolor[HTML]{EFEFEF} P6 & & & & & & & \\
        P7 & & & & & & & \\
        \rowcolor[HTML]{EFEFEF} P8 & & & & & & & \\
        P9 & & & & & & & \\
        \rowcolor[HTML]{EFEFEF} P10 & & & & & & & \\\hline
    \end{tabular}}
\end{table}

==> fig_tab/prompt_example.tex <==
\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/prompt_example.png}
    \caption{An actual example of our prompt and LLM output for text-to-gloss translation experiments. \rotem{I assume the input is part of the batches the model gets in the prompt? it should be reflected in the figure to show it's not an extra input to the LLM and how it is passed..}}
    \label{fig:prompt_example}
\end{figure}

==> fig_tab/system_overview.tex <==
\begin{teaserfigure}
    \centering
    \includegraphics[width=1\linewidth]{figures/hero_fig.png}
    \caption{Our system translates English text into a photorealistic ASL video with non-manual information. It starts with an English text input (first row), generates ASL tokens capturing both manual and non-manual details (second row), produces a skeletal pose sequence (third row), and finally creates the photorealistic ASL video (fourth row). \han{@all, please check the stylization.}}
    % \han{should we have a longer sentence? Ideally has 6-7 video frames. Still working on stylization...} \rotem{thinking about it again, instead of putting it here, I would have 1-2 examples here- only text->gloss->ours with expressions (or through pose), then have a no expression vs expression fig later on in the paper..}}
    \label{fig:system_overview}
\end{teaserfigure}

==> fig_tab/user_study_sec2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/user_study_sec2.png}
    \caption{\han{to add}}
    \label{fig:user_study_sec2}
\end{figure}

==> fig_tab/user_study_sec3.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> fig_tab/userstudy_ratings.tex <==
\begin{figure}[t]
    \centering
    \subfloat[Understanding ratings per sentence type.]{ \includegraphics[width=0.48\textwidth,valign=c]{figures/per_sentence_translation_ratings.png}
    \label{fig:per_sentence}}
    \subfloat[Semantic Translation Assessment.]{\includegraphics[width=0.35\textwidth,valign=c]{figures/translation_ratings.png}
    \label{fig:translation_ratings}}
    \caption{
% \todo{Update results and caption.} 
    Violin plots show estimated marginal means of translation ratings for each of the four video conditions. Translations of raw videos were rated significantly more accurate than all AI video conditions. Indicated on the figure, translations of AI (Full) and AI (w/o Expression) models were significantly more accurate than ratings of AI w/ annotation videos. Error bars show 95 percent confidence intervals. ** denotes p < .01.
    % Signed videos were generated using the following approaches: \textit{AI w/ Annotation} (leveraging human-annotated English-based glosses (manual markers) from the ASLLRP dataset, along with our manually annotated linguistic information (non-manual markers), as input for Modules 2 and 3 of our prototype system), \textit{Video Retargeting} (using skeletal poses from the ASLLRP dataset as inputs for Module 3), and \textit{AI w/ LLM} (our prototype system). All these approaches trained on the How2Sign dataset to generate the final signed output. In contrast, \textit{Raw Video} samples were directly taken from the ASLLRP dataset without additional processing or training.
    % \Description[This figure presents the results from two sections of our user study evaluating video quality. It contains two sub-figures. Each sub-figure displays the percentage of responses, with the right side (blue) representing better ratings and the left side (red) representing worse rating. The left sub-figure focused on visual and motion quality and the right sub-figure focused on translation quality. In the left sub-figure, it contains three questions: how easy is it to understand this video? Rate the visual quality of the signing in this video. Rate the naturalness of the motion. In the right sub-figure, it also contains three questions: is the meaning of the video the same as the English text? What is the quality of the translation? Take into account ASL grammar and style. How accurately does the facial expression match the English text?]}
    \label{fig:userstudyresults}
    }
\end{figure}



==> setup.tex <==
\usepackage{bm}
\usepackage{soul}
\usepackage{array}
% \usepackage{minted}
\usepackage{subfig}
\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{listings}
\lstset{
    basicstyle=\ttfamily,           % Use a monospaced font
    columns=fullflexible,           % Maintain alignment and spacing
    breaklines=true,                % Automatically break long lines
    breakatwhitespace=true,         % Break lines at whitespace
    linewidth=1\textwidth,        % Limit the line width to 80% of text width
    numbers=left,                   % Add line numbers on the left
    numberstyle=\tiny\color{gray},  % Style for line numbers
    stepnumber=1,                   % Number every line
    firstnumber=1,                  % Start line numbering at 1
    numbersep=5pt,                  % Space between line numbers and text
    frame=single,                   % Add a frame around the listing
    escapeinside={\%*}{*)},         % Allows LaTeX commands inside listings
    extendedchars=true,             % Supports extended characters
    literate={â}{{\^a}}1            % Example to handle specific extended characters
}
% \usepackage[table,xcdraw,dvipsnames]{xcolor} # original
% \usepackage{arydshln}
% \usepackage[export]{adjustbox}
% \usepackage{subfig}
\usepackage{subcaption}
\usepackage{hyperref}
\usepackage{verbatim}
\usepackage[nameinlink]{cleveref}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{minted}
% \usepackage{adjustbox}
% \usepackage{colortbl}
\usepackage{tabularx}
\usepackage{comment}
\usepackage{longtable}
\newcommand{\rev}[1]{\textcolor{black}{#1}}
% \definecolor{green}{rgb}{0.08, 0.47, 0.16}
% \definecolor{darkblue}{HTML}{0C0893} 
% \definecolor{brilliantlavender}{rgb}{0.6, 0.4, 0.8}
% \definecolor{candypink}{rgb}{0.89, 0.44, 0.48}
% \definecolor{lightpurple}{rgb}{0.8, 0.5, 0.98}
% \definecolor{green}{rgb}{0.08, 0.47, 0.16}
% \definecolor{violet}{rgb}{0.96, 0.5, 0.5}
% \definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
% \definecolor{darkpastelpurple}{rgb}{0.59, 0.44, 0.84}
% \definecolor{mediumslateblue}{rgb}{0.48, 0.41, 0.93}
\definecolor{RoyalBlue}{rgb}{0.48, 0.41, 0.93}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\sethlcolor{cyan}

\newcommand{\eg}{\textit{e.g.,\ }}
\newcommand{\ie}{\textit{i.e.,\ }}
\newcommand{\etal}{\textit{et al.\ }}
\newcommand{\etals}{\textit{et al's\ }}
% \newcommand{\participants}{\textcolor{red}{5} }
% \newcommand{\participants}{30\ } # original
% \newcommand{\nwoman}{24\ } # original
% \newcommand{\nman}{6\ } # original
% \newcommand{\removespace}{\vspace*{-0.25cm}}
% \newcommand{\nASLearlierthanten}{Three\ }
% \newcommand{\nASLbetweenten}{one\ }
% \newcommand{\nASLproficiencyexcelleent}{3\ } 
% \newcommand{\nASLproficiencygood}{1\ } 
% \newcommand{\nEGproficiencygood}{3\ }
% \newcommand{\nEGacceptable}{1\ }
% \newcommand{\nASLusedaily}{3\ }
% \newcommand{\nASLuseweekly}{1\ }
% \newcommand{\nEGdaily}{3\ }
% \newcommand{\nEGweekly}{1\ }

% \newcommand\han[1]{\textcolor{mediumslateblue}{han: #1}}
% \newcommand\rotem[1]{\textcolor{green}{rotem: #1}}
% \newcommand\colin[1]{\textcolor{purple}{colin: #1}}
% \newcommand\todo[1]{\textcolor{red}{todo: #1}}
% \newcommand\revise[1]{\textcolor{mediumslateblue}{#1}}
% \newcommand\toadd[1]{\textcolor{darkblue}{consider to add: #1}}


\newcommand\addauthornote[1]{%
  \if@ACM@anonymous\else
    \g@addto@macro\addresses{\@addauthornotemark{#1}}%
  \fi}

% \newcommand\@addauthornotemark[1]{\let\@tmpcnta\c@footnote
%    \setcounter{footnote}{#1}\addtocounter{footnote}{-1}
%     \g@addto@macro\@currentauthors{\footnotemark\relax\let\c@footnote\@tmpcnta}}
